Merging synthetic and real embryo data for advanced AI predictions

Accurate embryo morphology assessment is essential in assisted reproductive technology for selecting the most viable embryo. Artificial intelligence has the potential to enhance this process. However, the limited availability of embryo data presents challenges for training deep learning models. To address this, we trained two generative models using two datasets-one we created and made publicly available, and one existing public dataset-to generate synthetic embryo images at various cell stages, including 2-cell, 4-cell, 8-cell, morula, and blastocyst. These were combined with real images to train classification models for embryo cell stage prediction. Our results demonstrate that incorporating synthetic images alongside real data improved classification performance, with the model achieving 97% accuracy compared to 94.5% when trained solely on real data. This trend remained consistent when tested on an external Blastocyst dataset from a different clinic. Notably, even when trained exclusively on synthetic data and tested on real data, the model achieved a high accuracy of 92%. Furthermore, combining synthetic data from both generative models yielded better classification results than using data from a single generative model. Four embryologists evaluated the fidelity of the synthetic images through a Turing test, during which they annotated inaccuracies and offered feedback. The analysis showed the diffusion model outperformed the generative adversarial network, deceiving embryologists 66.6% versus 25.3% and achieving lower Frechet inception distance scores.

==> figures/FID_plots.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/plot_FID_GAN.png}
        \caption{StyleGAN2}
        \label{fig:plot1}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/plot_FID_LDM.png}
        \caption{LDM}
        \label{fig:plot2}
    \end{subfigure}
    \caption{FID scores over epochs for (a) StyleGAN and (b) LDM across the five embryo cell stages models: 2-cell, 4-cell, 8-cell, Blastocyst, and Morula.}
    \label{fig:FID_plots}
\end{figure}

==> figures/image_quality.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.7\linewidth]{images/image_quality.png}
\caption{Average responses from embryologists on the quality of the images they identified as fake.}
\label{fig:quality}
\end{figure}

==> figures/vgg_results.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{images/vgg_results.png}
\caption{Classification results for the VGG16 model on the test dataset (real images). The model was trained using various combinations of data sources, including StyleGAN, LDM, and real images, represented by the bars in the figure. Each combination highlights the impact of these data sources on the model's performance.}
\label{fig:vgg_results}
\end{figure}
